Towards Generalizable Agents in Text-Based Educational Environments: A Study of Integrating RL with LLMs

There has been a growing interest in developing learner models to enhance learning and teaching experiences in educational environments. However, existing works have primarily focused on structured environments relying on meticulously crafted representations of tasks, thereby limiting the agent's ability to generalize skills across tasks. In this paper, we aim to enhance the generalization capabilities of agents in open-ended text-based learning environments by integrating Reinforcement Learning (RL) with Large Language Models (LLMs). We investigate three types of agents: (i) RL-based agents that utilize natural language for state and action representations to find the best interaction strategy, (ii) LLM-based agents that leverage the model's general knowledge and reasoning through prompting, and (iii) hybrid LLM-assisted RL agents that combine these two strategies to improve agents' performance and generalization. To support the development and evaluation of these agents, we introduce PharmaSimText, a novel benchmark derived from the PharmaSim virtual pharmacy environment designed for practicing diagnostic conversations. Our results show that RL-based agents excel in task completion but lack in asking quality diagnostic questions. In contrast, LLM-based agents perform better in asking diagnostic questions but fall short of completing the task. Finally, hybrid LLM-assisted RL agents enable us to overcome these limitations, highlighting the potential of combining RL and LLMs to develop high-performing agents for open-ended learning environments.

==> Figures/RQ3.tex <==
\begin{figure*}[h]
    \centering    
    \includegraphics[width=\linewidth]{Figures/patient_vs_agent.png}
    \caption{\textbf{Performance of different agents in interaction with different patients.} From left to right, the plot illustrates the \textit{Post-test Performance Score} (accuracy in diagnoses), \textit{Trajectory Quality Score} (diagnostic conversation quality), and \textit{Combined Score} (overall efficacy in diagnostic conversations leading to correct diagnoses) for different agents in different patients' scenarios. Averages are from all scenarios related to each patient.}

    \label{fig:agents_vs_patients}
\end{figure*}
\begin{figure}[h]
    \centering
    \includegraphics[width=\linewidth]{Figures/causes10.png}
    \caption{The top 5 most difficult causes for the agents.}
    \label{fig:top_causes}
\end{figure}
\begin{figure}[h]
    \centering
    \includegraphics[width=\linewidth]{Figures/kqs10.png}
    \caption{The top 5 most missed Key Questions over all scenarios averaged for all agents.}
    \label{fig:top_qs}
\end{figure}
\begin{figure*}[t]
    \centering
    \includegraphics[width=\linewidth]{Figures/conversation.png}
    \caption{An example of conversations conducted by the DRRN and Suggestion-Assisted RL (SARL) agent with the patient with joint pains in the scenario with Osteoarthritis as the most probable cause.}
    \label{fig:conversation}
\end{figure*}

==> Tables/Table1.tex <==
\begin{table*}
\centering
\renewcommand{\arraystretch}{1.2}  % Provide more space between table rows, if you prefer
\caption{Some typical commands}
\begin{tabular}{ccl} \hline
Command&A Number&Comments\\ \hline
\texttt{{\char'134}alignauthor} & 100& Author alignment\\
\texttt{{\char'134}numberofauthors}& 200& Author enumeration\\
\texttt{{\char'134}table}& 300 & For tables\\
\texttt{{\char'134}table*}& 400& For wider tables\\ \hline\end{tabular}
\end{table*}
\begin{table}
\centering
\renewcommand{\arraystretch}{1.2}  % Provide more space between table rows, if you prefer
\caption{Frequency of Special Characters}
\begin{tabular}{ccl} \hline
Non-English or Math&Frequency&Comments\\ \hline
\O & 1 in 1,000& For Swedish names\\
$\pi$ & 1 in 5& Common in math\\
\$ & 4 in 5 & Used in business\\
$\Psi^2_1$ & 1 in 40,000& Unexplained usage\\
\hline\end{tabular}
\end{table}
